Proton-air cross section measurement with the ARGO-YBJ cosmic ray experiment

The proton-air cross section in the energy range 1-100 TeV has been measured by the ARGO-YBJ cosmic ray experiment. The analysis is based on the flux attenuation for different atmospheric depths (i.e. zenith angles) and exploits the detector capabilities of selecting the shower development stage by means of hit multiplicity, density and lateral profile measurements at ground. The effects of shower fluctuations, the contribution of heavier primaries and the uncertainties of the hadronic interaction models, have been taken into account. The results have been used to estimate the total proton-proton cross section at center of mass energies between 70 and 500 GeV, where no accelerator data are currently available.

==> 2009_04_authors.tex <==
\author{G. Aielli} 
\affiliation{Dipartimento di Fisica dell'Universit\`a ``Tor Vergata'' - via della Ricerca Scientifica 1 - 00133 Roma - Italy}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Tor Vergata - via della Ricerca Scientifica 1 - 00133 Roma - Italy}  
 
\author{C. Bacci} 
\affiliation{Dipartimento di Fisica dell'Universit\`a ``Roma Tre'' - via della Vasca Navale 84 - 00146 Roma - Italy}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Roma3 - via della Vasca Navale 84 - 00146 Roma - Italy}  
 
\author{B. Bartoli} 
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Napoli - Complesso Universitario di Monte Sant'Angelo - via Cintia - 80126 Napoli - Italy}  
\affiliation{Dipartimento di Fisica dell'Universit\`a di Napoli - Complesso Universitario di Monte Sant'Angelo - via Cintia - 80126 Napoli - Italy}  
 
\author{P. Bernardini} 
\affiliation{Dipartimento di Fisica dell'Universit\`a del Salento - via per Arnesano - 73100 Lecce - Italy}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Lecce - via per Arnesano - 73100 Lecce - Italy}  
 
\author{X.J. Bi} 
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China}  
 
\author{C. Bleve}  
\affiliation{Dipartimento di Fisica dell'Universit\`a del Salento - via per Arnesano - 73100 Lecce - Italy}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Lecce - via per Arnesano - 73100 Lecce - Italy}  
 
\author{P. Branchini}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Roma3 - via della Vasca Navale 84 - 00146 Roma - Italy}  
 
\author{A. Budano}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Roma3 - via della Vasca Navale 84 - 00146 Roma - Italy}   
 
\author{S. Bussino} 
\affiliation{Dipartimento di Fisica dell'Universit\`a ``Roma Tre'' - via della Vasca Navale 84 - 00146 Roma - Italy}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Roma3 - via della Vasca Navale 84 - 00146 Roma - Italy}  
 
\author{A.K. Calabrese Melcarne} 
\affiliation{Istituto Nazionale di Fisica Nucleare - CNAF - viale Berti-Pichat 6/2 - 40127 Bologna - Italy} 
 
\author{P. Camarri} 
\affiliation{Dipartimento di Fisica dell'Universit\`a ``Tor Vergata'' - via della Ricerca Scientifica 1 - 00133 Roma - Italy}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Tor Vergata - via della Ricerca Scientifica 1 - 00133 Roma - Italy}  
 
\author{Z. Cao} 
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China}  
 
\author{A. Cappa} 
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Torino - via P. Giuria 1 - 10125 Torino - Italy}  
\affiliation{Istituto di Fisica dello Spazio Interplanetario dell'Istituto Nazionale di Astrofisica - corso Fiume 4 - 10133 Torino - Italy}  
 
\author{R. Cardarelli}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Tor Vergata - via della Ricerca Scientifica 1 - 00133 Roma - Italy}  
 
\author{S. Catalanotti} 
\affiliation{Dipartimento di Fisica dell'Universit\`a di Napoli - Complesso Universitario di Monte Sant'Angelo - via Cintia - 80126 Napoli - Italy} 
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Napoli - Complesso Universitario di Monte Sant'Angelo - via Cintia - 80126 Napoli - Italy}  
  
\author{C. Cattaneo} 
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Pavia - via Bassi 6 - 27100 Pavia - Italy}  
 
\author{P. Celio} 
\affiliation{Dipartimento di Fisica dell'Universit\`a ``Roma Tre'' - via della Vasca Navale 84 - 00146 Roma - Italy}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Roma3 - via della Vasca Navale 84 - 00146 Roma - Italy}  
 
\author{S.Z. Chen} 
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China}  
 
\author{Y. Chen} 
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China}  
 
\author{N. Cheng} 
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China}  
 
\author{P. Creti} 
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Lecce - via per Arnesano - 73100 Lecce - Italy}  
 
\author{S.W. Cui}  
\affiliation{Hebei Normal University - Shijiazhuang 050016 - Hebei - China}  
 
\author{B.Z. Dai}  
\affiliation{Yunnan University - 2 North Cuihu Rd - 650091 Kunming - Yunnan - P.R. China}  
 
\author{G. D'Al\'{\i} Staiti} 
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Catania - Viale A. Doria 6 - 95125 Catania - Italy}  
\affiliation{Universit\`a degli Studi di Palermo - Dipartimento di Fisica e Tecnologie Relative - Viale delle Scienze - Edificio 18 - 90128 Palermo - Italy}  
 
\author{Danzengluobu} 
\affiliation{Tibet University - 850000 Lhasa - Xizang - P.R. China}  
 
\author{M. Dattoli} 
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Torino - via P. Giuria 1 - 10125 Torino - Italy}  
\affiliation{Istituto di Fisica dello Spazio Interplanetario dell'Istituto Nazionale di Astrofisica - corso Fiume 4 - 10133 Torino - Italy}  
\affiliation{Dipartimento di Fisica Generale dell'Universit\`a di Torino - via P. Giuria 1 - 10125 Torino - Italy}  
 
\author{I. De Mitri\footnote[4]{Corresponding author (e-mail: ivan.demitri@le.infn.it)}}  
%\thanks{Corresponding author (e-mail: ivan.demitri@le.infn.it)} 
%\email{ivan.demitri@le.infn.it} 
\affiliation{Dipartimento di Fisica dell'Universit\`a del Salento - via per Arnesano - 73100 Lecce - Italy}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Lecce - via per Arnesano - 73100 Lecce - Italy}  
 
\author{B. D'Ettorre Piazzoli}  
\affiliation{Dipartimento di Fisica dell'Universit\`a di Napoli - Complesso Universitario di Monte Sant'Angelo - via Cintia - 80126 Napoli - Italy} 
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Napoli - Complesso Universitario di Monte Sant'Angelo - via Cintia - 80126 Napoli - Italy}  
 
\author{M. De Vincenzi} 
\affiliation{Dipartimento di Fisica dell'Universit\`a ``Roma Tre'' - via della Vasca Navale 84 - 00146 Roma - Italy}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Roma3 - via della Vasca Navale 84 - 00146 Roma - Italy}  
 
\author{T. Di Girolamo}  
\affiliation{Dipartimento di Fisica dell'Universit\`a di Napoli - Complesso Universitario di Monte Sant'Angelo - via Cintia - 80126 Napoli - Italy} 
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Napoli - Complesso Universitario di Monte Sant'Angelo - via Cintia - 80126 Napoli - Italy}  
 
\author{X.H. Ding} 
\affiliation{Tibet University - 850000 Lhasa - Xizang - P.R. China}  
 
\author{G. Di Sciascio}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Tor Vergata - via della Ricerca Scientifica 1 - 00133 Roma - Italy}  
 
\author{C.F. Feng} 
\affiliation{Shandong University - 250100 Jinan - Shandong - P.R. China}  
 
\author{Zhaoyang Feng} 
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China} 
 
\author{Zhenyong Feng} 
\affiliation{South West Jiaotong University - 610031 Chengdu - Sichuan - P.R. China}  
 
\author{F. Galeazzi} 
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Roma3 - via della Vasca Navale 84 - 00146 Roma - Italy} 
 
\author{P. Galeotti} 
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Torino - via P. Giuria 1 - 10125 Torino - Italy}  
\affiliation{Dipartimento di Fisica Generale dell'Universit\`a di Torino - via P. Giuria 1 - 10125 Torino - Italy}  
 
\author{R. Gargana} 
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Roma3 - via della Vasca Navale 84 - 00146 Roma - Italy} 
 
\author{Q.B. Gou}  
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China} 
 
\author{Y.Q. Guo} 
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China} 
 
\author{H.H. He}  
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China} 
 
\author{Haibing Hu}  
\affiliation{Tibet University - 850000 Lhasa - Xizang - P.R. China} 
 
\author{Hongbo Hu}  
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China} 
 
\author{Q. Huang} 
\affiliation{South West Jiaotong University - 610031 Chengdu - Sichuan - P.R. China}  
 
\author{M. Iacovacci}  
\affiliation{Dipartimento di Fisica dell'Universit\`a di Napoli - Complesso Universitario di Monte Sant'Angelo - via Cintia - 80126 Napoli - Italy} 
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Napoli - Complesso Universitario di Monte Sant'Angelo - via Cintia - 80126 Napoli - Italy}  
 
\author{R. Iuppa}  
\affiliation{Dipartimento di Fisica dell'Universit\`a ``Tor Vergata'' - via della Ricerca Scientifica 1 - 00133 Roma - Italy}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Tor Vergata - via della Ricerca Scientifica 1 - 00133 Roma - Italy}  
 
\author{I. James} 
\affiliation{Dipartimento di Fisica dell'Universit\`a ``Roma Tre'' - via della Vasca Navale 84 - 00146 Roma - Italy}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Roma3 - via della Vasca Navale 84 - 00146 Roma - Italy}  
 
\author{H.Y. Jia}  
\affiliation{South West Jiaotong University - 610031 Chengdu - Sichuan - P.R. China}  
 
\author{Labaciren}  
\affiliation{Tibet University - 850000 Lhasa - Xizang - P.R. China} 
 
\author{H.J. Li}  
\affiliation{Tibet University - 850000 Lhasa - Xizang - P.R. China} 
 
\author{J.Y. Li}  
\affiliation{Shandong University - 250100 Jinan - Shandong - P.R. China}  
 
\author{X.X. Li} 
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China}  
 
\author{B. Liberti}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Tor Vergata - via della Ricerca Scientifica 1 - 00133 Roma - Italy} 
 
\author{G. Liguori}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Pavia - via Bassi 6 - 27100 Pavia - Italy}  
\affiliation{Dipartimento di Fisica Nucleare e Teorica dell'Universit\`a di Pavia - via Bassi 6 - 27100 Pavia - Italy}  
 
\author{C. Liu} 
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China}  
 
\author{C.Q. Liu} 
\affiliation{Yunnan University - 2 North Cuihu Rd - 650091 Kunming - Yunnan - P.R. China}  
 
\author{M.Y. Liu}  
\affiliation{Hebei Normal University - Shijiazhuang 050016 - Hebei - China} 
 
\author{J. Liu} 
\affiliation{Yunnan University - 2 North Cuihu Rd - 650091 Kunming - Yunnan - P.R. China}  
 
\author{H. Lu}  
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China} 
 
\author{X.H. Ma}  
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China} 
 
\author{G. Mancarella}  
\affiliation{Dipartimento di Fisica dell'Universit\`a del Salento - via per Arnesano - 73100 Lecce - Italy}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Lecce - via per Arnesano - 73100 Lecce - Italy}  
 
\author{S.M. Mari}  
\affiliation{Dipartimento di Fisica dell'Universit\`a ``Roma Tre'' - via della Vasca Navale 84 - 00146 Roma - Italy}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Roma3 - via della Vasca Navale 84 - 00146 Roma - Italy}  
 
\author{G. Marsella} 
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Lecce - via per Arnesano - 73100 Lecce - Italy}  
\affiliation{Dipartimento di Ingegneria dell'Innovazione - Universit\`a del Salento - 73100 Lecce - Italy}  
 
\author{D. Martello}  
\affiliation{Dipartimento di Fisica dell'Universit\`a del Salento - via per Arnesano - 73100 Lecce - Italy}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Lecce - via per Arnesano - 73100 Lecce - Italy}  
 
\author{S. Mastroianni}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Napoli - Complesso Universitario di Monte Sant'Angelo - via Cintia - 80126 Napoli - Italy}  
 
\author{X.R. Meng}  
\affiliation{Tibet University - 850000 Lhasa - Xizang - P.R. China} 
 
\author{P. Montini}  
\affiliation{Dipartimento di Fisica dell'Universit\`a ``Roma Tre'' - via della Vasca Navale 84 - 00146 Roma - Italy}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Roma3 - via della Vasca Navale 84 - 00146 Roma - Italy}  
 
\author{C.C. Ning} 
\affiliation{Tibet University - 850000 Lhasa - Xizang - P.R. China} 
 
\author{A. Pagliaro} 
\affiliation{Istituto di Astrofisica Spaziale e Fisica Cosmica di Palermo - Istituto Nazionale di Astrofisica - via Ugo La Malfa 153 - 90146 Palermo - Italy}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Catania - Viale A. Doria 6 - 95125 Catania - Italy}  
 
\author{M. Panareo} 
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Lecce - via per Arnesano - 73100 Lecce - Italy}  
\affiliation{Dipartimento di Ingegneria dell'Innovazione - Universit\`a del Salento - 73100 Lecce - Italy}  
 
\author{L. Perrone} 
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Lecce - via per Arnesano - 73100 Lecce - Italy}  
\affiliation{Dipartimento di Ingegneria dell'Innovazione - Universit\`a del Salento - 73100 Lecce - Italy}  
 
\author{P. Pistilli} 
\affiliation{Dipartimento di Fisica dell'Universit\`a ``Roma Tre'' - via della Vasca Navale 84 - 00146 Roma - Italy}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Roma3 - via della Vasca Navale 84 - 00146 Roma - Italy}  
 
\author{X.B. Qu}  
\affiliation{Shandong University - 250100 Jinan - Shandong - P.R. China}  
 
\author{E. Rossi}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Napoli - Complesso Universitario di Monte Sant'Angelo - via Cintia - 80126 Napoli - Italy}  
 
\author{F. Ruggieri}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Roma3 - via della Vasca Navale 84 - 00146 Roma - Italy}  
 
\author{L. Saggese}  
\affiliation{Dipartimento di Fisica dell'Universit\`a di Napoli - Complesso Universitario di Monte Sant'Angelo - via Cintia - 80126 Napoli - Italy} 
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Napoli - Complesso Universitario di Monte Sant'Angelo - via Cintia - 80126 Napoli - Italy}  
 
\author{P. Salvini} 
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Pavia - via Bassi 6 - 27100 Pavia - Italy}  
 
\author{R. Santonico}  
\affiliation{Dipartimento di Fisica dell'Universit\`a ``Tor Vergata'' - via della Ricerca Scientifica 1 - 00133 Roma - Italy}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Tor Vergata - via della Ricerca Scientifica 1 - 00133 Roma - Italy} 
 
\author{P.R. Shen} 
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China} 
 
\author{X.D. Sheng} 
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China} 
 
\author{F. Shi}  
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China} 
 
\author{C. Stanescu} 
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Roma3 - via della Vasca Navale 84 - 00146 Roma - Italy}  
 
\author{A. Surdo} 
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Lecce - via per Arnesano - 73100 Lecce - Italy}  
 
\author{Y.H. Tan}  
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China} 
 
\author{P. Vallania}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Torino - via P. Giuria 1 - 10125 Torino - Italy}  
\affiliation{Istituto di Fisica dello Spazio Interplanetario dell'Istituto Nazionale di Astrofisica - corso Fiume 4 - 10133 Torino - Italy}  
 
\author{S. Vernetto}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Torino - via P. Giuria 1 - 10125 Torino - Italy}  
\affiliation{Istituto di Fisica dello Spazio Interplanetario dell'Istituto Nazionale di Astrofisica - corso Fiume 4 - 10133 Torino - Italy}  
 
\author{C. Vigorito}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Torino - via P. Giuria 1 - 10125 Torino - Italy}  
\affiliation{Istituto di Fisica dello Spazio Interplanetario dell'Istituto Nazionale di Astrofisica - corso Fiume 4 - 10133 Torino - Italy}  
 
\author{B. Wang}  
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China} 
 
\author{H. Wang}  
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China} 
 
\author{C.Y. Wu}  
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China} 
 
\author{H.R. Wu}  
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China} 
 
\author{B. Xu}  
\affiliation{South West Jiaotong University - 610031 Chengdu - Sichuan - P.R. China}  
 
\author{L. Xue}  
\affiliation{Shandong University - 250100 Jinan - Shandong - P.R. China}  
 
\author{Y.X. Yan}  
\affiliation{Hebei Normal University - Shijiazhuang 050016 - Hebei - China}  
 
\author{Q.Y. Yang}  
\affiliation{Yunnan University - 2 North Cuihu Rd - 650091 Kunming - Yunnan - P.R. China}  
 
\author{X.C. Yang}  
\affiliation{Yunnan University - 2 North Cuihu Rd - 650091 Kunming - Yunnan - P.R. China}  
 
\author{A.F. Yuan}  
\affiliation{Tibet University - 850000 Lhasa - Xizang - P.R. China} 
 
\author{M. Zha}  
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China} 
 
\author{H.M. Zhang} 
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China} 
 
\author{JiLong Zhang}  
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China} 
 
\author{JianLi Zhang}  
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China} 
 
\author{L. Zhang} 
\affiliation{Yunnan University - 2 North Cuihu Rd - 650091 Kunming - Yunnan - P.R. China}  
 
\author{P. Zhang} 
\affiliation{Yunnan University - 2 North Cuihu Rd - 650091 Kunming - Yunnan - P.R. China} 
 
\author{X.Y. Zhang} 
\affiliation{Shandong University - 250100 Jinan - Shandong - P.R. China} 
 
\author{Y. Zhang} 
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China} 
 
\author{Zhaxisangzhu} 
\affiliation{Tibet University - 850000 Lhasa - Xizang - P.R. China} 
 
\author{X.X. Zhou} 
\affiliation{South West Jiaotong University - 610031 Chengdu - Sichuan - P.R. China} 
 
\author{F.R. Zhu} 
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China} 
 
\author{Q.Q. Zhu} 
\affiliation{Key Laboratory of Particle Astrophyics - Institute of High Energy Physics - Chinese Academy of Science - P.O. Box 918 - 100049 Beijing - P.R. China} 
 
\author{G. Zizzi} 
\affiliation{Dipartimento di Fisica dell'Universit\`a del Salento - via per Arnesano - 73100 Lecce - Italy}  
\affiliation{Istituto Nazionale di Fisica Nucleare - Sezione di Lecce - via per Arnesano - 73100 Lecce - Italy}

